OrthoNets: Orthogonal Channel Attention Networks

Designing an effective channel attention mechanism implores one to find a lossy-compression method allowing for optimal feature representation. Despite recent progress in the area, it remains an open problem. FcaNet, the current state-of-the-art channel attention mechanism, attempted to find such an information-rich compression using Discrete Cosine Transforms (DCTs). One drawback of FcaNet is that there is no natural choice of the DCT frequencies. To circumvent this issue, FcaNet experimented on ImageNet to find optimal frequencies. We hypothesize that the choice of frequency plays only a supporting role and the primary driving force for the effectiveness of their attention filters is the orthogonality of the DCT kernels. To test this hypothesis, we construct an attention mechanism using randomly initialized orthogonal filters. Integrating this mechanism into ResNet, we create OrthoNet. We compare OrthoNet to FcaNet (and other attention mechanisms) on Birds, MS-COCO, and Places356 and show superior performance. On the ImageNet dataset, our method competes with or surpasses the current state-of-the-art. Our results imply that an optimal choice of filter is elusive and generalization can be achieved with a sufficiently large number of orthogonal filters. We further investigate other general principles for implementing channel attention, such as its position in the network and channel groupings. Our code is publicly available at https://github.com/hady1011/OrthoNets/

==> tables/High_Dim_Results.tex <==
\begin{table}[htbp]
	\centering
	\caption{Effect high dimensional space on randomly initialized orthogonal channel attention filters using ResNet-50 trained on ImageNet.}
	\label{High_Dim_Effect}
    \begin{tabular}{lccc}
    	\toprule
    	Method        & Parameters & Location & Top-1 acc       \\
    	\hline
    	SENet \cite{SENet} &   28.07M   & After & 77.86          \\
    	OrthoNet      &   28.07M   & After &  78.47          \\
    	\rowcolor{tb_bg_color}
    	OrthoNet-MOD  &   \textbf{25.56M}   & Before &  \textbf{78.52}          \\
    	\bottomrule
    \end{tabular}
\end{table}

==> tables/Ortho_Effect.tex <==
\begin{table}[htbp]
	\centering
	\caption{Effect of Enforcing Orthogonality in channel attention filters using ResNet-34 trained on ImageNet.}
	\label{Ortho_Effect}
    \begin{tabular}{lccccccccccc}
    	\toprule
    	Method          & & & & & & & & & &   & Top-1 acc\\
    	\hline
    	Random          & & & & & & & & & &    &  74.34\\
    	GAP             & & & & & & & & & &    &  74.83\\
    	\rowcolor{tb_bg_color}
    	Orthogonal      & & & & & & & & & &    &  75.20\\
    	\bottomrule
    \end{tabular}
\end{table}


==> tables/Table_R.tex <==
\begin{table}[htbp]
	\centering
    \caption{Results of more runs}
	\label{T1}                                       
    \begin{tabular}{lccc}
	\toprule
	Method & Try # & T1 acc & T5 acc \\
	\hline
	OrthoNet-MOD-101 (old)    & 1 & 79.69 & 94.61 \\
    OrthoNet-MOD-101          & 2 & 79.69 & 94.80 \\
    OrthoNet-MOD-101          & 3 & 79.93 & 94.77 \\
    OrthoNet-MOD-151          & 1 & 80.13 & 95.02 \\
    \bottomrule
	\end{tabular}
\end{table}

\begin{table}[htbp]
	\centering
    \caption{OrthoNet 50 & 101 Downstream Task Runs}
	\label{T2}                                       
    \begin{tabular}{lccccccc}
	\toprule
	Architecture & Method & AP & $AP_{50}$ \\
	\hline
	OrthoNet-50    & FasterRCNN & 0.388 &0.598\\
    OrthoNet-101   & FasterRCNN & 0.407 &0.618\\
    \bottomrule
	\end{tabular}
\end{table}

\begin{table}[htbp]
	\centering
    \caption{FcaNet-50-MOD vs FcaNet-50 on Birds}
	\label{T3}                                       
    \begin{tabular}{lccc}
	\toprule
	Method & Trials & T1 acc\\
	\hline
	FcaNet-50-MOD    & 4 & 97.42 $\pm 0.08$ \\
    FcaNet-50-TS    & 1 & 97.60  \\
    \bottomrule
	\end{tabular}
\end{table}



==> tables/frequency_combination.tex <==

\begin{table}[htbp]
	\centering
	\caption{The results of using different numbers of frequency components on ImageNet with ResNet-50 backbone.}
	\label{combination}
	\begin{tabular}{ccc}
		\toprule
		Number    & Top-1 acc   & Top-5 acc  \\
		\midrule
		1   & 77.26     & 93.55\\
		2	& 78.40		& 94.07\\
		4	& 78.38		& 94.03\\
		8   & 78.33		& 94.06\\ 
		16 	& \textbf{78.52}  	& \textbf{94.14}\\
		32 	& 78.42  	& 94.10\\
		\bottomrule
	\end{tabular}
\end{table}



%\begin{table}[htbp]
%	\centering
%	\caption{The effects of different combinations of frequency components on the ImageNet dataset.}
%	\label{combination}
%	\begin{tabular}{ccc}
%		\toprule
%		Number    & Top-1 acc   & Top-5 acc  \\
%		\midrule
%		1   &  & \\
%		2	&  77.30 & 93.51\\
%		4	&  77.27 & 93.57\\
%		8   &  77.51 & 93.63\\ 
%		16 	&  77.17 & 93.53\\
%		32 	&  77.60 & 93.78\\
%		\bottomrule
%	\end{tabular}
%\end{table}

%\begin{table}[htbp]
%	\centering
%	\caption{The effects of different combinations of frequency components on the ImageNet dataset.}
%	\label{combination}
%	\begin{tabular}{ccc}
%		\toprule
%		Number    & Top-1 acc   & Top-5 acc  \\
%		\midrule
%		1   & 77.26 & 93.55\\
%		2	&  78.40 & 94.07\\
%		4	&  78.27 & 94.06\\
%		8   &  78.25 & 94.01\\ 
%		16 	&  78.26 & 94.12\\
%		32 	&  78.37 & 94.08\\
%		\bottomrule
%	\end{tabular}
%\end{table}
